Generalized Self-concordant Hessian-barrier algorithms

Many problems in statistical learning, imaging, and computer vision involve the optimization of a non-convex objective function with singularities at the boundary of the feasible set. For such challenging instances, we develop a new interior-point technique building on the Hessian-barrier algorithm recently introduced in Bomze, Mertikopoulos, Schachinger and Staudigl, [SIAM J. Opt. 2019 29(3), pp. 2100-2127], where the Riemannian metric is induced by a generalized self-concordant function. This class of functions is sufficiently general to include most of the commonly used barrier functions in the literature of interior point methods. We prove global convergence to an approximate stationary point of the method, and in cases where the feasible set admits an easily computable self-concordant barrier, we verify worst-case optimal iteration complexity of the method. Applications in non-convex statistical estimation and $L^{p}$-minimization are discussed to given the efficiency of the method.

==> AnalyticCenter.tex <==
%%% Analytic center
%----------------------------------------------------------------------
% !TEX root = ./Main.tex
%

Let $h\in\scrF_{M,\nu}(\scrC)$ for $\nu\in(2,4]$. Consider the linearly constrained minimization problem 
\begin{equation}\label{eq:AnalyticCenter}
\min\{h(x)\vert x\in\bar{\scrC},Ax=b\}
\end{equation}
In the literature on interior-point methods where $h$ is usually chosen to be a standard self-concordant barrier, a solution to the above program is known as the \emph{analytic center} of the domain $\scrX=\bar{\scrC}\cap\scrA$. Note that, due to the barrier like property of generalized self-concordant functions, if problem \eqref{eq:AnalyticCenter} admits a solution $x^{0}\in\scrX^{\circ}$ it must satisfy $\nabla h(x^{0})\in\scrA_{0}^{\bot}$. In this section we establish existence and uniqueness of the analytic center in case where $h$ is a generalized self-concordant function of order $\nu\in(2,4]$ and constant $M>0$. We assume that there exists $x\in\dom h$ such that $H(x)\succ 0$, and split the argument into several cases. This implies in particular, that $h$ is non-degenerate, meaning that its Hessian is non-singular on $\scrC=\dom h$. Hence, $h$ is strictly convex on $\scrC$, which immediately implies uniqueness of the solution to problem \eqref{eq:AnalyticCenter} once existence has been shown. The necessary and sufficient condition for $x^{0}$ to be a global minimizer is that 
\[
\nabla h(x^{0})\in\scrA_{0}^{\bot}. 
\]
We are going to deduce existence of solutions from the classical Weierstrass' Theorem (see e.g. \cite{Ber99}). Assume first that $\nu\in(3,4]$. Since $h$ is assumed to be coercive in this case and $\scrA$ is closed, existence of a minimizer follows. Hence, we now focus on $\nu\in(2,3]$, and start with the range $\nu\in(2,3)$. To that end, let us reformulate the problem as a non-smooth composite optimization problem 
\begin{align*}
\min_{x\in\Rn}\{\Phi(x):=h(x)+\delta_{\scrA}(x)\},
\end{align*}
where $\delta_{\scrA}(x)$ is the indicator function (in the sense of convex analysis) of the polyhedral set $\scrA$. Then, $\dom(\Phi)=\dom(h)\cap\scrA\subseteq\scrX$, and for each $r\in\R$, the set $\lev_{\Phi}(r):=\{x\in\Rn\vert\Phi(x)\leq r\}$ is equal to $\lev_{h}(r)\cap\scrA$. Let $x\in\dom(\Phi)$ be point where $H(x)\succ 0$, and consider the level let $\lev_{\Phi}(\Phi(x))=\scrL_{h}(h(x))\cap\scrA$. In order to show that problem \eqref{eq:AnalyticCenter} has a solution, we show that this level set is compact. Towards this end, choose an arbitrary $y\in\lev_{\Phi}(\Phi(x))=\lev_{h}(h(x))\cap\scrA$, so that $\Phi(y)=h(y)$ and $y\in\scrX$. Since
\[
\omega_{\nu}(-\metric_{\nu}(x,y))\norm{y-x}^{2}_{x}\leq h(y)-h(x)-\inner{\nabla h(x),y-x}\leq \omega_{\nu}(\metric_{\nu}(x,y))\norm{y-x}^{2}_{x},
\]
it follows hat 
\begin{align*}
h(x)\geq  h(y)&\geq h(x)+\inner{\nabla h(x),y-x}+\omega_{\nu}(-\metric_{\nu}(x,y))\norm{y-x}^{2}_{x},
\end{align*}
and consequently 
\begin{align*}
\inner{\nabla h(x),x-y}\geq \omega_{\nu}(-\metric_{\nu}(x,y))\norm{y-x}^{2}_{x}.
\end{align*}
By the Cauchy Schwarz inequality  
\begin{equation}\label{eq:main}
\norm{\nabla h(x)}^{\ast}_{x}\geq\omega_{\nu}(-d_{\nu}(x,y))\norm{y-x}_{x}. 
\end{equation}
Using the assumption that $H(x)\succ 0$, there exists $\sigma_{h}(x)>0$ such that 
\begin{align*}
\norm{y-x}_{x}\geq \sigma_{h}(x)^{1/2}\norm{y-x}_{2}\qquad\forall y\in\lev_{\Phi}(\Phi(x)). 
\end{align*}
Since $\metric_{\nu}(x,y)=M\frac{\nu-2}{2}\norm{y-x}^{3-\nu}_{2}\norm{y-x}^{\nu-2}_{x}$, we conclude 
\begin{align*}
\metric_{\nu}(x,y)\leq M\frac{\nu-2}{2}\sigma_{h}(x)^{-\frac{3-\nu}{2}}\norm{y-x}_{x}.
\end{align*}
Combining this estimate with the bound \eqref{eq:main}, we see 
\begin{align*}
\omega_{\nu}(-\metric_{\nu}(x,y))\norm{y-x}_{x}&\leq M\frac{\nu-2}{2}\sigma_{h}(x)^{-\frac{3-\nu}{2}}\norm{y-x}_{x}\omega_{\nu}(-\metric_{\nu}(x,y))\\
&\leq M\frac{\nu-2}{2}\sigma_{h}(x)^{-\frac{3-\nu}{2}}\norm{\nabla h(x)}^{\ast}_{x}.
\end{align*}
The mapping $t\mapsto \omega_{\nu}(-t)t$ is strictly increasing on $(0,\infty)$, and bounded from above by $\frac{\nu-2}{4-\nu}$. Hence, if $ M\frac{\nu-2}{2}\sigma_{h}(x)^{-\frac{3-\nu}{2}}\norm{\nabla h(x)}^{\ast}_{x}<\frac{\nu-2}{4-\nu}$, then the equation
\begin{align*}
\omega_{\nu}(-t)t-M\frac{\nu-2}{2}\sigma_{h}(x)^{-\frac{3-\nu}{2}}\norm{\nabla h(x)}^{\ast}_{x}=0
\end{align*}
has a unique solution $t^{\ast}(x)$. We conclude that $\metric_{\nu}(y,x)\leq t^{\ast}(x)$ for all $y\in\lev_{\Phi}(\Phi(x))$, and therefore 
\begin{align*}
\norm{y-x}_{2}\leq \frac{t^{\ast}(x)}{M \sigma_{h}(x)^{\frac{\nu-2}{2}}\frac{\nu-2}{2}}<\infty\qquad\forall y\in\lev_{\Phi}(\Phi(x)).
\end{align*}
This shows the boundedness of the level set $\lev_{\Phi}(\Phi(x))$. Furthermore, \eqref{eq:main} delivers the  bound 
\begin{align*}
\norm{\nabla h(x)}^{\ast}_{x}<\frac{2\sigma_{h}(x)^{\frac{3-\nu}{2}}}{(4-\nu)M}.
\end{align*}
We finally discuss the case where $\nu=3$. This is the standard self-concordant case, and solved in \cite[][Theorem 4.1.11]{NesConvex}. Using the fact that $\metric_{3}(x,y)=\frac{M}{2}\norm{y-x}_{x}$, inequality \eqref{eq:main} boils down to 
\begin{align*}
\frac{M}{2}\norm{\nabla h(x)}^{\ast}_{x}\geq \omega_{3}(-\metric_{3}(x,y))\metric_{3}(y,x).
\end{align*}
Arguing in the same way as in the previous case, it can be seen that if $\frac{M}{2}\norm{\nabla h(x)}^{\ast}_{x}<1$, the equation $\omega_{3}(-t)t-\frac{M}{2}\norm{\nabla h(x)}^{\ast}_{x}=0$ has a unique solution $t^{\ast}(x)$, implicitly defined by 
\begin{align*}
t^{\ast}(x)\left(1-\frac{M}{2}\norm{\nabla h(x)}^{\ast}_{x}\right)=\ln(1+t^{\ast}(x)). 
\end{align*}
This implies $\norm{y-x}_{2}\leq \frac{2 t^{\ast}(x)}{M\sqrt{\sigma_{h}(x)}}$ for all $y\in\lev_{\Phi}(\Phi(x))$, and therefore a minimizer exists. 




==> Center.tex <==
%----------------------------------------------------------------------
%%% Analytic center
%----------------------------------------------------------------------
% !TEX root = ./MainHBA_Potential.tex
%

For the construction of our algorithmic scheme it will be important to have access to a $\const$-analytic center, i.e. a point $x^{0}\in\scrX^{\circ}$ such that 
\begin{equation}\label{eq:h}
h(x)\geq h(x^{0})-\const\qquad\forall x\in\scrX. 
\end{equation}
To obtain such a point $x^{0}$, we need to be able to approximately solve the minimization problem 
\[
\min_{x\in\scrX}h(x). 
\]
This assumption is very common in potential reduction schemes \cite{Ye92,Ye98,HaeLiuYe18}. In case where $\scrX$ is bounded, existence of an exact analytic center is guaranteed and we can use any efficient solver for computing it. In the case where $\scrX$ is unbounded, existence of an exact analytic center is guaranteed if the classical existence condition given by the Weierstrass' theorem are satisfied. If $h\in\scrF_{M,\nu}(C)$ for $\nu\in (3,4]$ then by Definition \ref{def:bgk} the function $h$ is coercive, and therefore the program \eqref{eq:h} has a solution. In the remaining cases, where $\nu\in(2,3]$ we either have to assume that the feasible set is bounded or that there exists a point $x\in\scrX$ under which the dual norm $\norm{\nabla h(x)}^{\ast}_{x}$ is "small". We give precise conditions in Appendix \ref{app:analytic}, extending the discussion in \cite{SunTran18}. We just mention here that if problem \eqref{eq:h} has a solution, it must be unique, given the global non-degenericity of the Hessian $H(x)\succ 0$ on $C$. 


==> Experimental_Design.tex <==
%----------------------------------------------------------------------
%%% Example: Experimental Design
%----------------------------------------------------------------------
% !TEX root = ../MainHBA_Potential.tex
%

Given a sample $(s_{1},u_{1}),\ldots,(s_{m},u_{m})$, consider the problem of estimating a vector $\beta\in\Rn$ from experiments of the form 
\[
u_{i}=s_{i}^{\top}\beta+w_{i}\quad i=1,2,\ldots,m. 
\]
where $w_{i}$ is a measurement noise. Assume the vectors $w_{i}$ are independent Gaussian random variables with mean zero and unit variance, and the \emph{design matrix}
\[
S=\left[\begin{array}{c}
s_{1}^{\top}\\
\vdots\\
s_{m}^{\top}
\end{array}\right]\in\R^{m\times n}
\]
has rank $n$. The maximum likelihood estimator is the ordinary least squares estimator of the linear model given above, with solution 
\[
\hat{\beta}=(S^{\top}S)^{-1}S^{\top}u.
\]
Since $\hat{\beta}=\beta+(S^{\top}S)^{-1}S^{\top}w$, the associated residual vector $\hat{e}=\hat{\beta}-\beta$ has zero mean and covariance matrix $E=(S^{\top}S)^{-1}.$ The goal of \emph{experimental design} is to choose the vectors $s_{i}$ from among the possible choices so that the error covariance matrix $E$ is "small"; See e.g. \cite{BoyVan04} for an introduction. To state the optimal experimental design in its pure form, let us assume that the vectors $s_{1},\ldots,s_{m}$ can be drawn form a given set of covariates $v_{1},\ldots,v_{p}$ Let $m_{j}\geq 0$ denote the number of experiments for which $v_{j}$ is chosen as an active covariate. Then, the error covariance matrix can be expressed as 
\begin{align*}
E=(S^{\top}S)^{-1}=\left(\sum_{i=1}^{m}s_{i}s_{i}^{\top}\right)^{-1}=\left(\sum_{i=1}^{p}m_{i}v_{i}v_{i}^{\top}\right)^{-1}.
\end{align*}
The basic experimental design is thus the problem 
\begin{align*}
 & \min_{(m_{1},\ldots,m_{p})\in\N^{p}}  \left(\sum_{i=1}^{p}m_{i}v_{i}v_{i}^{\top}\right)^{-1}\\
 \text{s.t .} & m_{i}\geq 0,\sum_{i=1}^{p}m_{i}=m
 \end{align*}
In this original formulation, it is seen that the experimental design problem is a hard combinatorial optimization problem. In order to develop easy approximate solutions, various relaxation schemes have been proposed. One of the most successful ones is the $D$-optimal experiment design, in which we minimize the determinant of the error covariance matrix $E$. We can pose this problems as 
\begin{align*}
 & \min_{x\in\Rn} -\log\det\left(\sum_{j=1}^{p}x_{j}v_{j}v_{j}^{\top}\right)\\
\text{s.t.: } & x_{i}\geq 0,\sum_{i=1}^{p}x_{i}=1. 
\end{align*} 
Calling $V\in\R^{p\times n}$ the matrix consisting of all possible covariates available in our experiment, and assume that $\rank(V)=p<n$. Then, it can be shown that $f$ is twice continuously differentiable on the relative interior of the feasible set $\scrX=\Rn_{+}\cap\scrA$, where $\scrA=\{x\in\Rn\vert\mathds{1}^{\top}x=1\}$, with $\nabla f(x)=\diag(-C)$ and $\nabla^{2}f(x)=C\circ C$ (the Hadamard product), where $C=V^{\top}(VXV^{\top})^{-1}V$, and $X=\diag(x_{1},\ldots,x_{n})$. Note that $\dom(f)=\Rn_{++}$. As kernel generating distance we use the log-barrier $h(x)=-\sum_{i=1}^{n}\log(x_{i})$.  In \cite[][Section 2.2]{LuFreNes18} it is shown that $h-f$ is convex, so that $(f,h)$ is convex adaptable. 

==> Poisson.tex <==
%----------------------------------------------------------------------
%%% Example: Poisson Inverse
%----------------------------------------------------------------------
% !TEX root = ../Main.tex
%

In a variety of applications, ranging from nuclear medicine to night vision and from astronomy to traffic analysis, data are collected by counting a series of discrete events, such as photons hitting a detector or vehicles passing a sensor. The measurements are often inherently noisy due to low count levels, and we wish to reconstruct salient features of the
underlying phenomenon from these noisy measurements as accurately as possible. The inhomogeneous Poisson process model has been used effectively in many such contexts. In this model it is assumed that the number of counters follows a Poisson distribution $y\sim \Poi(m)$ with unknown mean and variance $m=Wx^{\ast}$, where $x^{\ast}\in\Rn_{+}$ is the signal or image of interest and $W\in\R^{m\times n}_{+}$ is a linear operator mapping a scene onto an $m$-dimensional set of observations. The task is to recover the true image $x^{\ast}$ based on the availability of a sample $y_{i}\sim \Poi(Wx^{\ast})$. Let $w_{i}\in\Rn$ denote the rows of the matrix $W$. We assume that $w_{i}\neq 0$ for all $i=1,2,\ldots,m$ and $\sum{i=1}^{m}w_{ij}>0$ for all $j=1,2,\ldots,m$, so that $w_{i}^{\top}x>0$ for all $i=1,2,\ldots,m$. This is a standard assumption in the literature \cite{VarShepKau85}. Following a maximum likelihood approach, the probability of observing a particular vector $y$ of counts is given by 
\[
p(y\vert Wx^{\ast})=\prod_{i=1}^{m}\frac{(w_{i}^{\top}x^{\ast})^{y_{i}}}{y_{i}!}\exp(-w_{i}^{\top}x^{\ast}). 
\]
The negative log-likelihood function is thus 
\begin{align*}
\sum_{i=1}^{m}w_{i}^{\top}x-\sum_{i=1}^{m}y_{i}\ln(w_{i}^{\top}x)+\sum_{i=1}^{m}\ln(y_{i}!).
\end{align*}
Neglecting the constant $\sum_{i=1}^{m}\ln(y_{i}!)$, and introducing the small regularization parameter $\eps>0$\footnote{Note that given the assumption that $w_{i}^{\top}x>0$ for all $1\leq i\leq m$, we do not need to introduce $\eps$ to make gradient evaluations well-posed, but rather to ensure numeric stability.}, we arrive at the maximum likelihood problem 
\begin{equation}
\max_{x\in\Rn_{+}}f_{0}(x):=\sum_{i=1}^{m}w_{i}^{\top}x-\sum_{i=1}^{m}y_{i}\ln(w_{i}^{\top}x+\eps)
\end{equation}
To make this problem well-posed we will assume that $w_{i}^{\top}x>0$ for all $x\in\Rn_{++}$. Furthermore, the dimension of the signal $x^{\ast}$ is typically much larger than the number of observations, so we are in a high-dimensional regime. Thus, there is a need to regularize the problem through an appropriate choice of penalty function incorporating the desired features of a solution. This leads to the composite optimization problem over the positive orthant
\begin{equation}\label{eq:f_Poisson}
\min_{x\in\Rn_{+}}f_{0}(x)+f_{1}(x),
\end{equation}
where $f_{1}(x)$ is a sparsity promoting penalty term. It is well known that $x\mapsto f_{0}(x)$ is convex, but not globally Lipschitz. To construct $\HBA(\mu,L)$, we use the Burg entropy $h\in\scrH_{2,3}(\Rn_{++})$, given by 
\[
h(x)=-\sum_{j=1}^{n}\ln(x_{j})
\]
From Lemma 7 in \cite{BauBolTeb16}, we know that $(f_{0},h)$ is $L$-smooth, with any $L\geq \norm{y}_{1}$, and the introduction of the regularizing factor $\eps>0$ in the loss function $f_{0}$ does not change this property. Assume that the penalty part in the composite formulation \eqref{eq:f_Poisson} is the $L_{p}$-norm $f_{1}(x)=\gamma \norm{x}^{p}_{p}=\sum_{i=1}^{n}\abs{x_{i}}^{p}$ for $p\in(0,1]$ and $\gamma>0$, a tuning parameter. We claim that the function $Lh-f$ is convex for any $L\geq 2\norm{y}_{1}$. To verify this claim, first observe that 
\begin{align*}
Lh-f=(\frac{L}{2}h-f_{0})+(\frac{L}{2}h-f_{1}).
\end{align*}
Now we distinguish two different cases. Assume first that $p\in(0,1)$. Then $f_{1}(x)$ is is concave, meaning that $\frac{L}{2}h-f_{1}$ is convex for any $L>0$.  Since $(f_{0},h)$ is $L$-smooth, the claim follows. Now, assume that $p=1$, so that $f_{1}(x)=\gamma\norm{x}_{1}$. For $x\in\Rn_{++}=C$, the function $\frac{L}{2}h(x)-f_{1}(x)$ is convex if and only if $\frac{L}{2}H(x)-\nabla^{2}f_{1}(x)\succ 0$. But, since $\nabla^{2}f_{1}(x)=0$ for all $x\in C$, the claim follows. 


%Therefore, running HBA with the potential function $F_{\mu}(x)=f(x)+\mu h(x)$ will be a potential decreasing method with optimal iteration complexity.

==> optimization.tex <==
%%% PROBLEM FORMULATION
%----------------------------------------------------------------------
% !TEX root = ./MainHBA_Potential.tex
%

\subsection{First-order optimality conditions}
\label{sec:optimality}
This section presents optimality conditions for solving problem \eqref{eq:P}, involving a potential function 
\begin{equation}
F_{\mu}(x)=f(x)+\mu h(x),
\end{equation}
where $\mu>0$ is a user-defined scaling parameter and $h\in\scrF_{M,\nu}(\scrC)$ for some $\nu\in(2,4]$. We will use this potential function to follow a classical interior penalty approach in deriving approximate first-order optimality condition for problem \eqref{eq:P}. To that end, we make the following geometric derivability assumption on the set of local solutions of \eqref{eq:P}.

\begin{assumption}\label{ass:approximate}
For every local solution $\bar{x}\in\scrX_{\ast}$ there exists a sequence $\{x^{k}\}_{k\geq 1}$ such that $\lim_{k\to\infty}x^{k}=\bar{x}$ and $x^{k}\in\scrX^{\circ}$ for all $k\geq 1$. 
\end{assumption}
This assumption is rather mild, and actually a standard one in interior-point methods \cite{Ber99}.


Let $x^{\ast}$ be an arbitrary local solution to \eqref{eq:P}. Take $\delta>0$ small enough so that the problem 
\begin{align*}
 \min_{x\in\Rn} & g(x):=f(x)+\frac{1}{4}\norm{x-x^{\ast}}^{4}_{2}\\
\text{s.t. } & x\in\scrX,\norm{x-x^{\ast}}_{2}\leq\delta
\end{align*}
has $x^{\ast}$ as its unique isolated solution. Let $\{\mu_{j}\}_{j\geq 1}$ be a sequence such that $\mu_{j}\to 0^{+}$. Given an approximate analytic center $x^{0}\in\scrX^{\circ}$, characterized in Appendix \ref{app:analytic}, define the function $\Phi_{j}:\Rn\to\R\cup\{+\infty\}$ by 
\begin{equation}
\Phi_{j}(x):=g(x)+\mu_{j}[h(x)-h(x^{0})].
\end{equation}
Since $h(x)\geq h(x^{0})-\const$ for all $x\in\dom(h)$, the problem 
\begin{equation}\label{eq:perturbed}
\min_{x}\Phi_{j}(x) \text{ s.t. }\norm{x-x^{\ast}}_{2}\leq\delta,\;Ax=b,
\end{equation}
has a solution $x_{j}$. Note that the introduction of the barrier-generating function $h$ absorbs the set constraint $x\in\bar{\scrC}$, and so we do not have to list this constraint explicitly anymore. Solving this problem for every $j\geq 1$, we obtain a sequence $\{x_{j}\}_{j\geq 1}$ satisfying $\norm{x_{j}-x^{\ast}}\leq \delta$ and $Ax_{j}=b$ for all $j\geq 1$. Hence, we can extract a converging subsequence, $\{x_{j}\}_{j\in\scrJ}\to \bar{x}$. We claim that $\bar{x}=x^{\ast}$, and argue via contradiction. Assume that $\bar{x}\neq x^{\ast}$. Observe that 
\[
\liminf_{j\to\infty,j\in\scrJ}\mu_{j}[h(x_{j})-h(x^{0})]\geq\liminf_{j\to\infty,j\in\scrJ}\mu_{j}\times (-C_{0})= 0,
\] 
and hence, 
\begin{align*}
\liminf_{j\to\infty,j\in\scrJ}\Phi_{j}(x_{j})=g(\bar{x})+\liminf_{j\to\infty,j\in\scrJ}\mu_{j}[h(x_{j})-h(x^{0})]\geq g(\bar{x}). 
\end{align*}

By Assumption \ref{ass:approximate}, there exists $\tilde{x}\in \scrX^{\circ}$ such that $\norm{\tilde{x}-x^{\ast}}_{2}\leq\delta$ and $g(\bar{x})>g(\tilde{x})\geq g(x^{\ast})$. \PD{I could not understand, why.} By definition of $x_{j}$, we deduce that 
\[
\Phi_{j}(x_{j})\leq \Phi_{j}(\tilde{x})\qquad \forall j\geq 1. 
\]
Consequently, \PD{I could not understand, why.}
\begin{align*}
\limsup_{j\to\infty,j\in\scrJ}\Phi_{j}(x_{j})\leq \limsup_{j\to\infty,j\in\scrJ}\Phi_{j}(\tilde{x})=g(\tilde{x}),
\end{align*}
and we must have $g(\bar{x})\leq g(\tilde{x})$, which is absurd. Since $\{x_{j}\}_{j\in\scrJ}$ is an arbitrary converging subsequence, we conclude that $x^{\ast}=\bar{x}$.\\ 

Next, observe that the first-order optimality condition for the point $x_{j}$ is the existence of a Lagrange multiplier $y_{j}\in\R^{m}$ such that 
\begin{align*}
A^{\top}y_{j}&=\nabla g(x_{j})+\mu_{j}\nabla h(x_{j})\\
&=\nabla F_{\mu_{j}}(x_{j})+(x_{j}-x^{\ast})\norm{x_{j}-x^{\ast}}^{2}_{2}. 
\end{align*}
Rearranging, this implies that 
\begin{equation}\label{eq:condition1}
\nabla F_{\mu_{j}}(x_{j})-A^{\top}y_{j}\to 0 \text{ as } j\to\infty.
\end{equation}
We distinguish two cases: Suppose first that $x^{\ast}\in\scrX^{\circ}$. In this case, for any sequence $\mu_{j}\downarrow 0$, we have $x_{j}\to x^{\ast}$, and $\mu_{j}\nabla h(x_{j})\to 0$. Hence, 
\[
\lim_{j\to\infty}\left(\nabla f(x_{j})-A^{\top}y_{j}\right)=0. 
\]
Next, we assume hat $x^{\ast}\in\bd(\scrX)=\bd(\bar{\scrC})\cap\scrA$. We need the following basic technical fact derived from the structure of generalized self-concordant functions.\\


\PD{It seems that this paragraph is the same as on page 13.} Let $h\in\scrF_{M,\nu}(\scrC)$ and $x_{j}\to \bd(\scrC)=\bar{\scrC}\setminus \scrC$. Then $h(x_{j})\to\infty$. We claim that this implies $\norm{\nabla h(x_{j})}_{2}\to\infty$. Indeed, by convexity, for all $y\in \scrC$, we have 
\begin{align*}
h(y)\geq h(x_{j})+\inner{\nabla h(x_{j}),y-x_{j}}. 
\end{align*}
Hence, 
\begin{align*}
\frac{h(y)-h(x_{j})}{\norm{\nabla h(x_{j})}_{2}}\geq \inner{\frac{\nabla h(x_{j})}{\norm{\nabla h(x_{j})}_{2}},y-x_{j}}\geq -\norm{y-x_{j}}_{2}.
\end{align*}
Therefore, 
\begin{align*}
h(y)\geq h(x_{j})-\norm{y-x_{j}}\cdot\norm{\nabla h(x_{j})}_{2}
\end{align*}
If $\norm{\nabla h(x_{j})}_{2}$ would be bounded, the right-hand side diverges to $\infty$, whereas the left hand side is bounded for $y\in\dom (h)$. This gives a contradiction. We conclude that $h$ is \emph{Legendre:} 
\begin{equation}\label{eq:legendre}
x_{j}\to x^{\ast}\in \bd(\scrC)\Rightarrow \norm{\nabla h(x_{j})}_{2}\to\infty. 
\end{equation} 
Based on this, we can deduce the following result which coincides with Lemma 4.2 in \cite{ABB04}. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{lemma}\label{lem:normal}
Let $\{x_{j}\}_{j\geq 1}\subset \scrC$ be such that $x_{j}\to x^{\ast}\in\bd(\scrC)=\bar{\scrC}\setminus \scrC$. and $\frac{\nabla h(x_{j})}{\norm{\nabla h(x_{j})}}\to p\in\Rn$ with $h\in\scrF_{M,\nu}(\scrC)$. Then $p\in \NC_{\bar{\scrC}}(x^{\ast})=\{p\in\Rn\vert \inner{p,y-x^{\ast}}\leq 0\; \forall y\in\bar{\scrC}\}$.
\end{lemma}
\begin{proof}
By convexity of $h$, $\inner{\nabla h(x_{j})-\nabla h(y),x_{j}-y}\geq 0$ for all $y\in \scrC$. Dividing by $\norm{\nabla h(x_{j})}$ and letting $j\to\infty$, we get $\inner{p,y-x^{\ast}}\leq 0$ for all $y\in \scrC$, which holds also for $y\in\bar{\scrC}$. Hence, $p\in \NC_{\bar{\scrC}}(x^{\ast})$. 
\end{proof}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Let us choose $\mu_{j}=\frac{1}{\norm{\nabla h(x_{j})}_{2}}$ \PD{I think, we can't choose $\mu$ in this way since $x_j$ is defined by $\mu$.}, we conclude first by \eqref{eq:legendre} that $\mu_{j}\to 0$ as $j\to\infty$, and second, by Lemma \ref{lem:normal}, that $\mu_{j}\nabla h(x_{j})\to p\in\NC_{\bar{\scrC}}(x^{\ast})$. Hence, 
\begin{align*}
\lim_{j\to\infty}\left(\nabla f(x_{j})-A^{\top}y_{j}\right)=-p\in-\NC_{\bar{\scrC}}(x^{\ast}). 
\end{align*}
This implies in turn, for all $\eps>0$ and all $x\in\scrX$ for $j$ sufficiently large, it must be 
\begin{equation}
\inner{\nabla f(x_{j}),x-x_{j}}\geq-\eps. 
\end{equation}

Furthermore, \eqref{eq:condition1} implies that for all $\eps>0$ we can choose $j$ sufficiently large so that 
\begin{align*}
\norm{\nabla f(x_{j})-A^{\top}y_{j}+\mu_{j}\nabla h(x_{j})}_{\infty}\leq\eps. 
\end{align*}
Therefore, 
\begin{align*}
-\eps H(x_{j})^{-1/2}\1&-\mu_{j}H(x_{j})^{-1/2}\nabla h(x_{j})\leq H(x_{j})^{-1/2}\left(\nabla f(x_{j})-A^{\top}y_{j}\right)\\
&\leq \eps H(x_{j})^{-1/2}\1-\mu_{j}H(x_{j})^{-1/2}\nabla h(x_{j}),
\end{align*}
so that 
\begin{align*}
\norm{\nabla f(x_{j})-A^{\top}y_{j}}^{\ast}_{x_{j}}&\leq\eps \norm{\1}_{x_{j}}^{\ast}+\mu\norm{\nabla h(x_{j})}^{\ast}_{x_{j}}\\
&\leq \eps \sqrt{n}\frac{1}{\sigma_{\min}(x_ {j})^{1/2}}+\mu_{j}\norm{\nabla h(x_{j})}^{\ast}_{x_{j}},
\end{align*}
where we used that 
\begin{align*}
\norm{\1}_{x}^{\ast}&=\sqrt{\inner{H(x)^{-1}\1,\1}}=\norm{H(x)^{-1/2}\1}_{2}\leq \sqrt{\tr(H(x)^{-1})}\cdot\norm{\1}_{2}\\
&\leq \sqrt{\frac{n}{\sigma_{\min}(x)}}.
\end{align*}
where $\sigma_{\min}(x)$ is the smallest eigenvalue of the matrix $H(x)\succ 0$. Since $\scrC$ contains no lines, by Lemma \ref{lem:nondeg} we have $H(x_{j})\succ 0$ for all $j\geq 1$. Hence, there exists $\underline{\sigma}>0$ such that $\sigma_{\min}(x_{j})\geq \underline{\sigma}$ for all $j$, and we conclude that  
\begin{align*}
\norm{\nabla f(x_{j})-A^{\top}y_{j}}^{\ast}_{x_{j}}&\leq\eps\sqrt{\frac{n}{\underline{\sigma}}}+\mu_{j}\norm{\nabla h(x_{j})}^{\ast}_{x_{j}}. 
\end{align*}
By definition \ref{def:kgd}(c), the sequence $\{\mu_{j}\norm{\nabla h(x_{j})}^{\ast}_{x_{j}}\}_{j\geq 1}$ converges to 0. Summarizing all these findings, we propose the following Definition for approximate stationary points of problem \eqref{eq:Opt}.
%%%%%
\begin{definition}\label{def:KKT}
Given $\eps>0$, a point $x\in\scrX^{\circ}$ is called an $\eps$-KKT point for \eqref{eq:Opt} if there exists $y\in\R^{m}$ such that 
\begin{itemize}
\item[(KKT1)] $\inner{\nabla f(x),w-x}\geq-\eps$ for all $w\in\scrX$, and% \PD{Shouldn't it be $\inner{\nabla f(x) + A^{\top}y,w-x}\geq-\eps$?}\MS{ If $w,x\in\scrX$ then by definition $A(w-x)=0$.}
\item[(KKT2)] $\norm{\nabla f(x)-A^{\top}y}_{x}^{\ast}\leq\eps.$
\end{itemize}
\end{definition}
\PD{We obtain this Definition 3.2 as a corollary of the
fact that $\lim_{j\to\infty}\left(\nabla f(x_{j})-A^{\top}y_{j}\right)=0$. Then why don’t we use the inequality
$\|\nabla f(x_{j})-A^{\top}y_{j}\|_2 \leq \varepsilon$ as a definition of $\varepsilon$-KKT point?}

\begin{remark}
It is interesting to remark what the above conditions apply for the very important special case in which $\bar{\scrC}=\Rn_{+}$ and $h(x)=-\sum_{i=1}^{n}\log(x_{i})$ is the log-barrier. In this case, the Riemannian metric is generated by the Hessian matrix $H(x)=X^{-2}:=\diag\{x_{1}^{-2},\ldots,x_{n}^{-2}\}$. In this case condition (KKT1) can be seen as a condition that $-\nabla f(x)$ is close to the normal cone $\scrA_{0}^{\top}$. Condition (KKT2) reduces to the complementarity condition 
\begin{align*}
\norm{X(\nabla f(x)-A^{\top}y)}_{\infty}\leq \norm{\nabla f(x)-A^{\top}y}^{\ast}_{x}\leq \eps. 
\end{align*}
Both conditions are very similar to the $\eps$-KKT definition given in \cite{HaeLiuYe18}.
\end{remark}


%
%Based on the above construction, we can also derive conditions for a second-order $\eps$-KKT point. That that end, observe that for every $x\in\scrX^{\circ}$ at which $f$ is twice differentiable, we have 
%\begin{align*}
%\nabla^{2}\Phi_{j}(x)=\nabla^{2}f(x)+\mu_{j}H(x^{j})+\norm{x-x^{\ast}}^{2}\Id+2(x-x^{\ast})(x-x^{\ast})^{\top}.
%\end{align*}
%Therfore, for $x_{j}$ to be a local minimum of the perturbed problem \eqref{eq:perturbed}, a necessaray second order condition is that 
%\begin{align*}
%d^{\top}\left(\nabla^{2}f(x_{j})+\mu_{j}H(x^{j})+\norm{x-x^{\ast}}^{2}\Id+2(x-x^{\ast})(x-x^{\ast})^{\top}\right)d\geq 0.
%\end{align*}
%for all $d\in\scrA_{0}$. Define the symmetric positive definite matrix 
%\[
%M_{j}:=2(x_{j}-x^{\ast})(x_{j}-x^{\ast})^{\top}+\norm{x_{j}-x^{\ast}}^{2}\Id,
%\]
%and call $\delta_{j}=\sigma_{\max}(M_{j})$ the largest eigenvalue of $M_{j}$. Then we know that $\delta_{j}\to 0$ and and $d^{\top}M_{j}d\leq\delta_{j}\norm{d}_{2}^{2}$ for all $j\geq %1$. We thus arrive at the second-order necessary condition 
%\begin{align*}
%0\leq d^{\top}\left(\nabla^{2}f(x_{j})+\mu_{j}H(x_{j})+\delta_{j}\Id\right)d \quad\forall d\in\scrA_{0}. 
%\end{align*}
%Since $\mu_{j},\delta_{j}\to 0$ as $j\to\infty$, this suggests the following natural definition.
%%%%%%%%%%%%%%%%%%%%
%\begin{definition}\label{def:KKT2}
%Given $\eps>0$. Let $x\in\scrX^{\circ}$ be a point at which $f$ is twice continuously differentiable. $x$ is called an $\eps$-KKT2 point if there exists $y\in\R^{m}$ such that 
%\begin{enumerate}
%\item $\inner{\nabla f(x),w-x}\geq-\eps$ for all $w\in\scrX$,
%\item $\norm{\nabla f(x)-A^{\top}y}^{\ast}_{x}\leq\eps$,
%\item For all $d\in\scrA_{0}$ we have 
%\begin{equation}
%d^{\top}\left(\nabla^{2}f(x)+\mu H(x)+\eps\Id\right)d\geq 0. 
%\end{equation}
%\end{enumerate}
%\end{definition}


